DOSnet as a Non-Black-Box PDE Solver: When Deep Learning Meets Operator Splitting

Deep neural networks (DNNs) recently emerged as a promising tool for analyzing and solving complex differential equations arising in science and engineering applications. Alternative to traditional numerical schemes, learning-based solvers utilize the representation power of DNNs to approximate the input-output relations in an automated manner. However, the lack of physics-in-the-loop often makes it difficult to construct a neural network solver that simultaneously achieves high accuracy, low computational burden, and interpretability. In this work, focusing on a class of evolutionary PDEs characterized by having decomposable operators, we show that the classical ``operator splitting'' numerical scheme of solving these equations can be exploited to design neural network architectures. This gives rise to a learning-based PDE solver, which we name Deep Operator-Splitting Network (DOSnet). Such non-black-box network design is constructed from the physical rules and operators governing the underlying dynamics contains learnable parameters, and is thus more flexible than the standard operator splitting scheme. Once trained, it enables the fast solution of the same type of PDEs. To validate the special structure inside DOSnet, we take the linear PDEs as the benchmark and give the mathematical explanation for the weight behavior. Furthermore, to demonstrate the advantages of our new AI-enhanced PDE solver, we train and validate it on several types of operator-decomposable differential equations. We also apply DOSnet to nonlinear Schr\"odinger equations (NLSE) which have important applications in the signal processing for modern optical fiber transmission systems, and experimental results show that our model has better accuracy and lower computational complexity than numerical schemes and the baseline DNNs.

==> content/abstract.tex <==
\begin{abstract}
Deep neural networks (DNNs) recently emerged as a promising tool for analyzing and solving complex differential equations arising in science and engineering applications. Alternative to traditional numerical schemes, learning-based solvers utilize the representation power of DNNs to approximate the input-output relations in an automated manner. However, the lack of physics-in-the-loop often makes it difficult to construct a neural network solver that simultaneously achieves high accuracy, low computational burden, and interpretability. In this work, focusing on a class of evolutionary PDEs characterized by having decomposable operators, we show that the classical ``operator splitting'' numerical scheme of solving these equations can be exploited to design neural network architectures. This gives rise to a learning-based PDE solver, which we name Deep Operator-Splitting Network (DOSnet). Such non-black-box network design as constructed from the physical rules and operators governing the underlying dynamics contains learnable parameters and is thus more flexible than the standard operator splitting scheme. Once trained, it enables the fast solution of the same type of PDEs. To demonstrate the advantages of our new AI-enhanced PDE solver, we train and validate it on several types of operator-decomposable differential equations which include linear PDEs and nonlinear reaction-diffusion equations as benchmarks, as well as nonlinear Schr\"odinger equations (NLSE) which finds applications in the signal processing for modern optical fiber transmission systems.
\end{abstract}



==> content/code.tex <==
\section{Code}
Here we show the pytorch-style code of DOSnet for Allen-Cahn model. 
\begin{itemize}
    \item \textit{class Nonlinear\_AC} defines the nonlinear operator from PDE.
    \item \textit{class OSB} defines the operator splitting block.
    \item \textit{class DOSnet} shows the whole structure of DOSnet.
\end{itemize}
\lstset{style=mystyle}
\begin{lstlisting}[language=Python]

class Nonlinear_AC(nn.Module):
  def __init__(self,features,dt):
    super(Nonlinear_AC, self).__init__()
    self.dt = torch.Tensor([dt]).cuda()

  def forward(self,input):
    B,C,H,W = input.shape
    out = input/(torch.sqrt(torch.exp(-2*self.dt)+\
                            (1-torch.exp(-2*self.dt))*input**2+1e-8))
    return out
    
class OSB(nn.Module):
    def __init__(self,in_channels,out_channels,features,kernel_size,dt):
        super(OSB, self).__init__()
        pad = int((kernel_size-1)/2)
        self.conv0 = nn.Conv2d(in_channels=in_channels, out_channels=features, \
                               kernel_size=kernel_size,padding= (pad,pad),\
                               padding_mode='circular', bias=False)
        self.conv1 = nn.Conv2d(in_channels=features, out_channels=out_channels,\
                               kernel_size=kernel_size,padding= (pad,pad),\
                               padding_mode='circular', bias=False)
        self.act = Nonlienar_AC(features,dt)
        for m in self.modules():
            if isinstance(m, nn.Conv2d):
                torch.nn.init.orthogonal_(m.weight.data)

    def forward(self,input):
        out = self.conv0(input)
        out = self.act(out)

        out = self.conv1(out)
        out = self.act(out)
        return out

class DOSnet(nn.Module):
    def __init__(self,num_of_layers,features,dt):
        super(DOSnet, self).__init__()
        kernel_size = 11
        pad = int((kernel_size-1)/2)
        layers = []
        for i in range(num_of_layers):
            layers.append(OSB(in_channels=1, out_channels=1,\
                              features = features, \
                              kernel_size=kernel_size,\
                              dt = dt))
        self.dosnet = nn.Sequential(*layers)

    def forward(self, input):
        x = input
        seq = []
        seq.append(input)
        for layer in self.dosnet:
            x_previous = x.view(x.shape[0],-1)
            x = layer(x)
            mul = torch.mean(x_previous*x.view(x.shape[0],-1),\
                             axis = 1).view(-1,1,1,1)
            x = x*torch.sign(mul)
            seq.append(x)
        return x,seq
\end{lstlisting}

==> content/def_code.tex <==
%New colors defined below
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

%Code listing style named "mystyle"
\lstdefinestyle{mystyle}{
  backgroundcolor=\color{backcolour}, commentstyle=\color{codegreen},
  keywordstyle=\color{magenta},
  numberstyle=\tiny\color{codegray},
  stringstyle=\color{codepurple},
  basicstyle=\ttfamily\footnotesize,
  breakatwhitespace=false,         
  breaklines=true,                 
  captionpos=b,                    
  keepspaces=true,                 
  numbers=left,                    
  numbersep=5pt,                  
  showspaces=false,                
  showstringspaces=false,
  showtabs=false,                  
  tabsize=2
}

==> content/related_works.tex <==
\section{Related Works}
Although the idea of utilizing neural networks to solve differential equations is itself not new \cite{lee_neural_1990,yentis_vlsi_1996,lagaris_artificial_1998}, connecting deep learning with PDE has (re)emerged over the past few years. %past years, more and more works are emerging as the interdisciplinary area of DNN and PDE. 
Some are to reveal structural connections between DNN and continuous dynamical systems, such as \cite{e_proposal_2017,Lizhen2017,chang2018}. More works are to solve PDEs using DNN as a tool.
%Recently, it becomes a hot research topic again, especially in the community of applied mathematics.
Many works utilize the approximation universality of DNN and use it as ansatz of solutions \cite{cybenko_approximation_1989,hornik_multilayer_1989,yarotsky18a,yarotsky_phase_2019,gao_efficient_2017,raissi_physics-informed_2019,sirignano_dgm_2018,han_solving_2019,beck_deep_2019}. The DNN based solution ansatz is plugged into PDEs, which are iteratively trained by enforcing equality constraints of PDE.
%then the DNNs are expected to converge to true solutions. 
Another type of approach utilizes the relationship between PDE and stochastic differential equation (SDE). \cite{e_deep_2017} converts the PDE problem as a stochasitc control problem of and uses DNN to approximate the policy function. \cite{beck_deep_2019} uses operator splitting to simplify the problem before applying DNN to approximate solutions. \cite{beck_machine_2019} extend the method of SDE to fully-nonlinear PDEs. Instead of fixing the PDE and learning its solution, one can also directly learning the PDE itself.
\cite{long_pde-net_2018,long_pde-net_2019} apply Euler discretization and approximate PDEs by residual neural networks \cite{he_deep_2016}. 

Different from the existing paradigm, our approach is to learn the evolution flow of PDEs instead of the solutions or equations directly. We propose DOSnet which is characterized by the composition of a sequence of learnable evolution operators, each of which can be seen as a flexible version of the classical operator splitting numerical scheme. Some earlier works also contain the idea of evolution operator or use operator splitting technique together with deep learning. For example, 
\cite{Lizhen2017} interprets DNN with evolution flow of ODE and linear transport equation.
\cite{alecsa_new_2020,liu_toward_2018}
developed DNN-based operator splitting optimization algorithms.
\cite{beck_deep_2019} also use operator splitting in their PDE solver, but in a different approach. \cite{hager_deep_2018,fan_advancing_2020} employed neural networks for nonlinear compensation in optical fiber, which implicitly contain some idea of operator splitting and can be viewed as specific application of our general method.
Those work did not consider an adaptive-step learning strategy, which we found to play a key role in our method to reduce the complexity of the network.

